Solar chemical composition

The Sun is one of the fundamental benchmarks in astronomy, and there is ever growing interest in precise and accurate determinations of its chemical composition. We present the current state-of-the-art in spectroscopic determinations of the solar elemental abundances, that now routinely employ three-dimensional (3D) radiative-hydrodynamic simulations of the solar photosphere and post-processing in non-local thermodynamic equilibrium (non-LTE). We critically review the recent literature and present recommended present-day and protosolar abundances of the 83 long-lived elements, and discuss their implications vis-\`a-vis primitive meteorites, helioseismology, neutrino fluxes, and the Solar Modelling Problem.

==> table/abundances.tex <==
\begin{table}[htbp]
\caption{Recommended abundances for $83$ long-lived elements in the present-day solar convective envelope. Based on spectroscopy of the quiet solar photosphere informed by 3D non-LTE (``3N'), 3D LTE (``3L'), or 3D LTE with non-LTE versus LTE abundance corrections based on 1D or \mtd{} model atmospheres (``3L+1N'), for $58$ elements from lithium to thorium (\sect{resultslight} to \sect{resultsheavy}); other elements are discussed in \sect{resultsother}, and the protosolar nebula is discussed in \sect{discussionproto}.}
\label{tab:abundances}
\begin{tabular*}{\textwidth}{@{}lllr|lllr@{}}
\toprule
Z & Elem. & Note & $\lgeps{X}$ &
Z & Elem. & Note & $\lgeps{X}$ \\
\midrule
 1 &  H &            Reference & $  12$  & 47 & Ag &                   3N & $    1.15\pm   0.08$  \\ 
 2 & He &      Helioseismology & $  10.934\pm  0.010$  & 48 & Cd &                CI-Tc & $    1.66\pm   0.03$  \\ 
 3 & Li &                   3N & $    0.96\pm   0.06$  & 49 & In &              Sunspot & $    0.80\pm   0.20$  \\ 
 4 & Be &                   3N & $    1.21\pm   0.05$  & 50 & Sn &                   3L & $    2.02\pm   0.10$  \\ 
 5 &  B &                3L+1N & $    2.70\pm   0.20$  & 51 & Sb &                CI-Tc & $    1.01\pm   0.07$  \\ 
 6 &  C &                   3N & $    8.47\pm   0.04$  & 52 & Te &                CI-Tc & $    2.14\pm   0.02$  \\ 
 7 &  N &                   3N & $    7.84\pm   0.07$  & 53 &  I &                CI-Tc & $    1.66\pm   0.17$  \\ 
 8 &  O &                   3N & $    8.70\pm   0.04$  & 54 & Xe &              Nuclear & $    2.26\pm   0.06$  \\ 
 9 &  F &              Sunspot & $    4.40\pm   0.25$  & 55 & Cs &                CI-Tc & $    1.03\pm   0.03$  \\ 
10 & Ne &      Transition/Wind & $    8.07\pm   0.05$  & 56 & Ba &                   3N & $    2.27\pm   0.05$  \\ 
11 & Na &                   3N & $    6.22\pm   0.03$  & 57 & La &                   3L & $    1.12\pm   0.04$  \\ 
12 & Mg &                   3N & $    7.56\pm   0.03$  & 58 & Ce &                   3L & $    1.58\pm   0.04$  \\ 
13 & Al &                   3N & $    6.43\pm   0.03$  & 59 & Pr &                   3L & $    0.75\pm   0.05$  \\ 
14 & Si &                   3N & $    7.55\pm   0.04$  & 60 & Nd &                   3L & $    1.42\pm   0.04$  \\ 
15 &  P &                3L+1N & $    5.35\pm   0.04$  & 61 & Pm &             Unstable &   \\ 
16 &  S &                   3N & $    7.06\pm   0.04$  & 62 & Sm &                   3L & $    0.95\pm   0.04$  \\ 
17 & Cl &              Sunspot & $    5.31\pm   0.20$  & 63 & Eu &                   3N & $    0.49\pm   0.05$  \\ 
18 & Ar &                 Wind & $    6.38\pm   0.10$  & 64 & Gd &                   3L & $    1.08\pm   0.04$  \\ 
19 &  K &                   3N & $    5.07\pm   0.03$  & 65 & Tb &                   3L & $    0.31\pm   0.10$  \\ 
20 & Ca &                   3N & $    6.30\pm   0.03$  & 66 & Dy &                   3L & $    1.10\pm   0.04$  \\ 
21 & Sc &                3L+1N & $    3.13\pm   0.04$  & 67 & Ho &                   3L & $    0.48\pm   0.11$  \\ 
22 & Ti &                   3L\footnotemark[1] & $    4.97\pm   0.05$  & 68 & Er &                   3L & $    0.93\pm   0.05$  \\ 
23 &  V &                3L+1N & $    3.90\pm   0.08$  & 69 & Tm &                   3L & $    0.11\pm   0.04$  \\ 
24 & Cr &                   3L\footnotemark[1] & $    5.65\pm   0.04$  & 70 & Yb &                   3L & $    0.85\pm   0.11$  \\ 
25 & Mn &                   3N\footnotemark[2] & $    5.47\pm   0.08$  & 71 & Lu &                   3L & $    0.10\pm   0.09$  \\ 
26 & Fe &                   3N & $    7.46\pm   0.04$  & 72 & Hf &                   3L & $    0.86\pm   0.05$  \\ 
27 & Co &                3L+1N & $    4.94\pm   0.07$  & 73 & Ta &                CI-Tc & $   -0.14\pm   0.02$  \\ 
28 & Ni &                   3L & $    6.20\pm   0.05$  & 74 &  W &                   3L & $    0.79\pm   0.11$  \\ 
29 & Cu &                3L+1N & $    4.18\pm   0.05$  & 75 & Re &                CI-Tc & $    0.29\pm   0.02$  \\ 
30 & Zn &                3L+1N & $    4.56\pm   0.05$  & 76 & Os &                   3L & $    1.31\pm   0.12$  \\ 
31 & Ga &                   3L & $    3.02\pm   0.05$  & 77 & Ir &                CI-Tc & $    1.32\pm   0.03$  \\ 
32 & Ge &                   3L & $    3.62\pm   0.10$  & 78 & Pt &                CI-Tc & $    1.60\pm   0.03$  \\ 
33 & As &                CI-Tc & $    2.29\pm   0.04$  & 79 & Au &                   3L & $    0.91\pm   0.12$  \\ 
34 & Se &                CI-Tc & $    3.32\pm   0.02$  & 80 & Hg &                CI-Tc & $    1.04\pm   0.16$  \\ 
35 & Br &                CI-Tc & $    2.55\pm   0.10$  & 81 & Tl &              Sunspot & $    0.92\pm   0.17$  \\ 
36 & Kr &         Wind/nuclear & $    3.19\pm   0.10$  & 82 & Pb &                3L+1N & $    1.95\pm   0.08$  \\ 
37 & Rb &                3L+1N & $    2.34\pm   0.08$  & 83 & Bi &                CI-Tc & $    0.61\pm   0.03$  \\ 
38 & Sr &                3L+1N & $    2.84\pm   0.07$  & 84 & Po &             Unstable &   \\ 
39 &  Y &                   3N & $    2.29\pm   0.07$  & 85 & At &             Unstable &   \\ 
40 & Zr &                   3L\footnotemark[1] & $    2.59\pm   0.05$  & 86 & Rn &             Unstable &   \\ 
41 & Nb &                   3L & $    1.47\pm   0.06$  & 87 & Fr &             Unstable &   \\ 
42 & Mo &                   3L & $    1.88\pm   0.09$  & 88 & Ra &             Unstable &   \\ 
43 & Tc &             Unstable &   & 89 & Ac &             Unstable &   \\ 
44 & Ru &                   3L & $    1.75\pm   0.08$  & 90 & Th &                3L+1N & $    0.03\pm   0.10$  \\ 
45 & Rh &                   3N\footnotemark[3] & $    1.06\pm   0.18$  & 91 & Pa &             Unstable &   \\ 
46 & Pd &                   3L & $    1.57\pm   0.11$  & 92 &  U &                CI-Tc & $   -0.52\pm   0.04$  \\ 
\botrule
\end{tabular*}
\footnotetext[1]{Full weight given to lines of \ion{Ti}{II}, \ion{Cr}{II}, and \ion{Zr}{II}, that show small non-LTE effects.}
\footnotetext[2]{A mean of two studies, one of which uses 3D non-LTE modelling.}
\footnotetext[3]{An approximate 3D non-LTE versus 3D LTE abundance correction for the \ion{Rh}{I} UV resonance lines has been applied based on calculations for \ion{Ag}{I} UV resonance lines.}
\end{table}


==> table/meteorites.tex <==
\begin{table}[htbp]
\caption{Abundances of CI chondrites converted to the scale of the present-day solar convective envelope with our recommended photospheric abundances (see \sect{discussiontcond}). 50\% condensation temperatures $T_{\mathrm{c}}$ taken from \citet{2019AmMin.104..844W}.  Last column gives predicted abundance corrections $\Delta\lgeps{X}$ needed to remove the trend with $50\%$ condensation temperature (\fig{fig:tcond}) that extends down to $T_{\mathrm{c}}=495\,\mathrm{K}$; for elements with $240\leq T_{\mathrm{c}}<495\,\mathrm{K}$, $\Delta\lgeps{X}$ is capped at $-0.06\,\dex$. The corrected abundances $\lgeps{X}+\Delta\lgeps{X}$ are incorporated into our final recommendations for the $15$ elements discussed in \sect{resultsother} (labelled ``CI-Tc'' in \tab{tab:abundances}).}
\label{tab:meteorites}
\begin{tabular*}{\textwidth}{@{}lrrrr|lrrrr@{}}
\toprule
Z & Elem. & $\lgeps{X}$ & $T_{\mathrm{c}} / K$ & $\Delta\lgeps{X}$  &
Z & Elem. & $\lgeps{X}$ & $T_{\mathrm{c}} / K$ & $\Delta\lgeps{X}$  \\
\midrule
 1 &  H & $   8.20\pm   0.04$ &   &   & 47 & Ag & $   1.21\pm   0.04$ & $ 699$ & $ -0.047$  \\ 
 2 & He & $   1.29\pm   0.04$ &   &   & 48 & Cd & $   1.72\pm   0.03$ & $ 502$ & $ -0.060$  \\ 
 3 & Li & $   3.26\pm   0.02$ & $1148$ & $ -0.017$  & 49 & In & $   0.77\pm   0.03$ & $ 492$ & $ -0.060$  \\ 
 4 & Be & $   1.33\pm   0.03$ & $1551$ & $  0.010$  & 50 & Sn & $   2.08\pm   0.05$ & $ 604$ & $ -0.053$  \\ 
 5 &  B & $   2.77\pm   0.06$ & $ 740$ & $ -0.044$  & 51 & Sb & $   1.04\pm   0.07$ & $ 890$ & $ -0.034$  \\ 
 6 &  C & $   7.43\pm   0.08$ &   &   & 52 & Te & $   2.19\pm   0.02$ & $ 665$ & $ -0.049$  \\ 
 7 &  N & $   6.08\pm   0.21$ &   &   & 53 &  I & $   1.72\pm   0.17$ & $ 390$ & $ -0.060$  \\ 
 8 &  O & $   8.40\pm   0.01$ & $ 183$ &   & 54 & Xe & $  -1.94\pm   0.04$ &   &   \\ 
 9 &  F & $   4.62\pm   0.09$ & $ 674$ & $ -0.048$  & 55 & Cs & $   1.08\pm   0.03$ & $ 593$ & $ -0.054$  \\ 
10 & Ne & $  -1.12\pm   0.04$ &   &   & 56 & Ba & $   2.18\pm   0.03$ & $1423$ & $  0.002$  \\ 
11 & Na & $   6.27\pm   0.05$ & $1035$ & $ -0.024$  & 57 & La & $   1.19\pm   0.02$ & $1615$ & $  0.015$  \\ 
12 & Mg & $   7.53\pm   0.02$ & $1343$ & $ -0.004$  & 58 & Ce & $   1.59\pm   0.02$ & $1454$ & $  0.004$  \\ 
13 & Al & $   6.43\pm   0.03$ & $1652$ & $  0.017$  & 59 & Pr & $   0.77\pm   0.02$ & $1550$ & $  0.010$  \\ 
14 & Si & $   7.51\pm   0.02$ & $1314$ & $ -0.006$  & 60 & Nd & $   1.46\pm   0.02$ & $1630$ & $  0.016$  \\ 
15 &  P & $   5.44\pm   0.04$ & $1287$ & $ -0.007$  & 61 & Pm &  & &  \\ 
16 &  S & $   7.14\pm   0.04$ & $ 672$ & $ -0.049$  & 62 & Sm & $   0.95\pm   0.02$ & $1545$ & $  0.010$  \\ 
17 & Cl & $   5.24\pm   0.07$ & $ 472$ & $ -0.060$  & 63 & Eu & $   0.53\pm   0.02$ & $1491$ & $  0.006$  \\ 
18 & Ar & $  -0.54\pm   0.04$ &   &   & 64 & Gd & $   1.06\pm   0.02$ & $1630$ & $  0.016$  \\ 
19 &  K & $   5.08\pm   0.03$ & $ 993$ & $ -0.027$  & 65 & Tb & $   0.32\pm   0.02$ & $1630$ & $  0.016$  \\ 
20 & Ca & $   6.29\pm   0.03$ & $1535$ & $  0.009$  & 66 & Dy & $   1.14\pm   0.02$ & $1630$ & $  0.016$  \\ 
21 & Sc & $   3.04\pm   0.03$ & $1541$ & $  0.010$  & 67 & Ho & $   0.47\pm   0.02$ & $1630$ & $  0.016$  \\ 
22 & Ti & $   4.90\pm   0.03$ & $1565$ & $  0.011$  & 68 & Er & $   0.93\pm   0.02$ & $1630$ & $  0.016$  \\ 
23 &  V & $   3.95\pm   0.03$ & $1370$ & $ -0.002$  & 69 & Tm & $   0.13\pm   0.02$ & $1630$ & $  0.016$  \\ 
24 & Cr & $   5.63\pm   0.02$ & $1291$ & $ -0.007$  & 70 & Yb & $   0.93\pm   0.02$ & $1528$ & $  0.009$  \\ 
25 & Mn & $   5.48\pm   0.04$ & $1123$ & $ -0.018$  & 71 & Lu & $   0.10\pm   0.03$ & $1630$ & $  0.016$  \\ 
26 & Fe & $   7.45\pm   0.02$ & $1338$ & $ -0.004$  & 72 & Hf & $   0.71\pm   0.03$ & $1720$ & $  0.022$  \\ 
27 & Co & $   4.87\pm   0.02$ & $1354$ & $ -0.003$  & 73 & Ta & $  -0.15\pm   0.02$ & $1546$ & $  0.010$  \\ 
28 & Ni & $   6.21\pm   0.01$ & $1363$ & $ -0.002$  & 74 &  W & $   0.67\pm   0.05$ & $1736$ & $  0.023$  \\ 
29 & Cu & $   4.25\pm   0.05$ & $1034$ & $ -0.024$  & 75 & Re & $   0.26\pm   0.02$ & $1736$ & $  0.023$  \\ 
30 & Zn & $   4.61\pm   0.03$ & $ 704$ & $ -0.046$  & 76 & Os & $   1.35\pm   0.01$ & $1806$ & $  0.027$  \\ 
31 & Ga & $   3.07\pm   0.03$ & $1010$ & $ -0.026$  & 77 & Ir & $   1.31\pm   0.03$ & $1566$ & $  0.011$  \\ 
32 & Ge & $   3.60\pm   0.03$ & $ 830$ & $ -0.038$  & 78 & Pt & $   1.60\pm   0.03$ & $1370$ & $ -0.002$  \\ 
33 & As & $   2.30\pm   0.04$ & $1235$ & $ -0.011$  & 79 & Au & $   0.81\pm   0.04$ & $ 967$ & $ -0.029$  \\ 
34 & Se & $   3.37\pm   0.02$ & $ 701$ & $ -0.047$  & 80 & Hg & $   1.10\pm   0.16$ & $ 240$ & $ -0.060$  \\ 
35 & Br & $   2.61\pm   0.10$ & $ 420$ & $ -0.060$  & 81 & Tl & $   0.77\pm   0.04$ & $ 365$ & $ -0.060$  \\ 
36 & Kr & $  -2.27\pm   0.04$ &   &   & 82 & Pb & $   2.03\pm   0.03$ & $ 495$ & $ -0.060$  \\ 
37 & Rb & $   2.36\pm   0.02$ & $ 752$ & $ -0.043$  & 83 & Bi & $   0.67\pm   0.03$ & $ 480$ & $ -0.060$  \\ 
38 & Sr & $   2.90\pm   0.02$ & $1548$ & $  0.010$  & 84 & Po &  & &  \\ 
39 &  Y & $   2.16\pm   0.04$ & $1551$ & $  0.010$  & 85 & At &  & &  \\ 
40 & Zr & $   2.53\pm   0.03$ & $1722$ & $  0.022$  & 86 & Rn &  & &  \\ 
41 & Nb & $   1.40\pm   0.04$ & $1561$ & $  0.011$  & 87 & Fr &  & &  \\ 
42 & Mo & $   1.93\pm   0.05$ & $1520$ & $  0.008$  & 88 & Ra &  & &  \\ 
43 & Tc &  & &  & 89 & Ac &  & &  \\ 
44 & Ru & $   1.76\pm   0.03$ & $1533$ & $  0.009$  & 90 & Th & $   0.05\pm   0.05$ & $1630$ & $  0.016$  \\ 
45 & Rh & $   1.04\pm   0.02$ & $1370$ & $ -0.002$  & 91 & Pa &  & &  \\ 
46 & Pd & $   1.66\pm   0.02$ & $1330$ & $ -0.004$  & 92 &  U & $  -0.53\pm   0.04$ & $1609$ & $  0.014$  \\ 
\botrule
\end{tabular*}
\end{table}

